Amortized Conditional Normalized Maximum Likelihood: Reliable Out of Distribution Uncertainty Estimation

While deep neural networks provide good performance for a range of challenging tasks, calibration and uncertainty estimation remain major challenges, especially under distribution shift. In this paper, we propose the amortized conditional normalized maximum likelihood (ACNML) method as a scalable general-purpose approach for uncertainty estimation, calibration, and out-of-distribution robustness with deep networks. Our algorithm builds on the conditional normalized maximum likelihood (CNML) coding scheme, which has minimax optimal properties according to the minimum description length principle, but is computationally intractable to evaluate exactly for all but the simplest of model classes. We propose to use approximate Bayesian inference technqiues to produce a tractable approximation to the CNML distribution. Our approach can be combined with any approximate inference algorithm that provides tractable posterior densities over model parameters. We demonstrate that ACNML compares favorably to a number of prior techniques for uncertainty estimation in terms of calibration on out-of-distribution inputs.

==> broader_impact.tex <==
\section{Broader Impact}
% tldr; uncertainty representation very important for real world decision-making. cite some practical domains where confidence measures and OOD detection are useful.

Models that can understand when their predictions may be wrong are essential to deploying machine learning for real-world decision making. 
No matter how well a model does on a training data, the real world inevitably provides anomalous situations that differ in some way from the training set such where such the model's predictions become unreliable. 
In domains like autonomous driving or medical diagnosis, where an incorrect prediction can lead to potentially disastrous consequences, it is better to have a system that can alert the user when its predictions should not be trusted rather than proceed overconfidently. 
We believe our approach is a step towards having systems that are able to reliably identify when they are likely to be mistaken, which would help to enable the deployment of powerful machine learning tools in risk-sensitive domains. 

That being said, our method is a tool that can potentially aid in applying machine learning in a wide variety of tasks, including tasks that would be harmful to society. 
This is not specific to our method, nor to just work on providing uncertainty estimates for machine learning, but rather a danger that all researchers who work on general, widely applicable techniques should keep in mind.

A more specific danger of systems that provide uncertainty estimates is that they could instill overconfidence in the uncertainty estimates instead. 
Take current (semi)-autonomous vehicles. 
The human driver would still be monitoring the situation around the vehicle and generally be ready to take control over the vehicle.
However, if the driver had been assured that the autonomous driving system would let the driver know when intervention is needed, the driver would be much more tempted to not be paying attention. 
Given that uncertainty estimation will never be perfect, if the system fails silently, the driver would be in much more danger than if he or she were paying attention and ready to intervene.
Thus, it is important for us as researchers to understand the limits of our methods, as well as making sure the users do as well.
%%SL.6.4: This is very well written!

% remark on positive and negative impacts are the same as other work on improving probabilsitic inference

==> extra_material.tex <==
% Old data table with STL10 data
\begin{table}
\centering
\scalebox{.7}{
\begin{tabular}{|c|ccc|ccc|}
			\hline 
			\multicolumn{1}{|c}{} & \multicolumn{3}{|c}{CIFAR10} & \multicolumn{3}{|c|}{STL10 (OOD Transfer)}\\
			\hline
			VGG16 & NLL & Accuracy  & ECE & OOD NLL & OOD Accuracy & OOD ECE \\ 
			\hline 
			ACNML (ours) & $0.2180\pm0.0041$ & $93.23\pm 0.09$ & $0.0246\pm0.0010$ & $\textbf{1.1118}\pm0.0145$ & $71.62\pm0.10$ & $\textbf{0.0776}\pm0.0030$\\ 
			% \hline 
			MAP (SWA) & $0.2694\pm0.0056$ & $93.23\pm0.13$  & $0.0430\pm0.0010$ & $1.3787\pm0.0245$ & $71.65\pm0.46$ & $0.2058\pm0.0044$\\ 
			% \hline 
			SWAG & $0.2257\pm0.0047$ & $93.31\pm0.04$ & $0.0284\pm0.0002$ & $1.2133\pm0.01999$ & $71.68\pm0.37$ & $0.1710\pm0.0037$ \\ 
			Full SWAG & $\textbf{0.2016} \pm 0.0031$ & $93.60 \pm 0.10$ & $0.0158 \pm 0.0030$ & $\textbf{1.1402} \pm 0.0342$  &    $72.19 \pm 0.06$ & $0.1463 \pm 0.0075$ \\
			% \hline
			% Marginal Likelihood (SWAG) & 0.2056 & 0.9337 & 0.0258 & 0.9941& 0.7190 & 0.1104 \\ 
			% \hline
			SWA-Dropout & $0.2328 \pm .0049$ & $93.23 \pm 0.36$ & $0.0284\pm0.0036$ & $1.3133 \pm 0.0000$ & $71.45 \pm 0.11$ & $0.1803 \pm 0.0024$\\
			% \hline
			SWA-Temp & $0.2481 \pm 0.0245$ & $93.61\pm 0.11$ & $0.0366 \pm 0.0063$ & $1.4082 \pm 0.0506$ & $71.92 \pm 0.01$ & $0.2089 \pm 0.0055$\\
			SGD & $0.3285\pm0.0139$ & $93.17\pm0.14$ & $0.0483\pm0.0022$ & $1.6528\pm0.039$ & $72.42\pm0.07$ & $0.2149\pm0.0027$ \\
			KFAC-Laplace & $0.2252\pm0.0032$ & $92.65\pm0.20$ & $\textbf{0.0094}\pm 0.0005$  & - & - & - \\
			SGLD & $\textbf{0.2001}\pm0.0059$ & $93.55\pm0.15$ & $\textbf{0.0082}\pm0.0012$  & - & - & -\\
			\hline
			\multicolumn{7}{|c|}{}\\
			\hline 
			WideResNet28x10 & NLL & Accuracy & ECE & OOD NLL & OOD Accuracy & OOD ECE\\ 
			\hline 
			% Amortized cNML (ours) & 0.1412 & 0.9640 & 0.8596 & 0.7693 & 0.045 & 0.023 \\ with temp 1.0
			ACNML (ours) & $0.1130\pm 0.0012$ & $96.38 \pm 0.03$ & $0.0122\pm 0.0006$ & $0.9279 \pm 0.0061$ & $76.90 \pm 0.11$ &  $\textbf{0.0821}\pm 0.0009$ \\ % temp 0.5
			% \hline 
			MAP (SWA) & $0.1128 \pm 0.0014$ & $96.41\pm0.01$ & $0.0099 \pm 0.0004$ & $1.0582\pm 0.0075$ & $76.93\pm 0.13$ &  $0.1349\pm 0.0021$\\ 
			% \hline 
			SWAG & $0.1125 \pm 0.0012$  &$96.28\pm 0.04$ & $\textbf{0.0042} \pm  0.0003$ & $1.0027\pm 0.0074$ & $76.58 \pm 0.01$ &  $0.1201 \pm 0.005$ \\ 
			Full SWAG &$ 0.1122 \pm 0.0009$ & $96.32 \pm 0.08$ & $0.0088 \pm 0.0006$ & $\textbf{0.8710} \pm 0.0000$ & $77.09 \pm 0.00$ & $0.1017 \pm 0.0000$\\
			% \hline
			SWA-Dropout & $0.1094 \pm 0.0021$ & $96.39 \pm 0.09$ & $0.0094 \pm 0.0014$ & $0.9914 \pm 0.0000$ & $76.91 \pm 0.00$ & $0.1421 \pm 0.0000$\\
			% Marginal Likelihood (SWAG) & 0.1445 & 0.9573 & 0.8894 & 0.755 & 0.0315 & 0.0471\\ 
			% \hline
			% \hline
			SWA-Temp & $\textbf{0.1064} \pm 0.0004$ & $96.46 \pm 0.04$ & $0.0080 \pm 0.0007$ & $0.9706 \pm 0.0000$ & $77.50 \pm 0.00$ & $0.1371 \pm 0.0000$ \\
			SGD & $0.1294\pm0.0022$ & $96.41 \pm 0.10$ & $0.0166 \pm 0.0007$ & $1.1308 \pm 0.0000$ & $76.75 \pm 0.00$ & $0.1561 \pm 0.0000$\\
			KFAC-Laplace & $0.1210\pm0.0020$ & $96.17 \pm 0.00$ & $0.0060 \pm 0.0003$& - & - & -\\
			SGLD & $0.1289 \pm 0.0009$ & $95.89 \pm 0.02$ & $0.0192 \pm 0.0007 $ & - & - & - \\
			\hline 
		\end{tabular} 
        }
\caption{\textbf{Expanded comparisons for ACNML}: Results for SWA-Dropout, SWA-Temp, SGD, KFAC-Laplace, SGLD, and Full-SWAG are taken from \citet{Maddox2019ALearning}. \todo{add our own versions of Full SWAG, add to the pruned table too}}
\label{tab:nll-acc-ece-expanded}
\end{table}


\begin{table*}
\centering
\scalebox{.7}{
\begin{tabular}{|c|ccc|}
			\hline 
			\multicolumn{1}{|c}{} & \multicolumn{3}{|c|}{STL10 (OOD Transfer)}\\
			\hline
			VGG16 & OOD NLL & OOD Accuracy & OOD ECE \\ 
			\hline 
			ACNML (ours) & $\textbf{0.7156}\pm0.0061 & $78.73\pm0.29 & $\textbf{0.0345}\pm0.0035$ \\ 
			% \hline 
			MAP (SWA) &  $0.9314\pm 0.0153$ & $78.74\pm0.35$ & $0.1464\pm0.0042$\\ 
			% \hline 
			SWAG & $0.7924\pm 0.0074$ & $78.83\pm0.28$ & $0.1152\pm0.0035$ \\ 
			\hline
			\multicolumn{4}{|c|}{}\\
			\hline 
			WideResNet28x10 & OOD NLL & OOD Accuracy & OOD ECE\\ 
			\hline 
			% Amortized cNML (ours) & 0.1412 & 0.9640 & 0.8596 & 0.7693 & 0.045 & 0.023 \\ with temp 1.0
			ACNML (ours) &  $\textbf{0.4477} \pm 0.0044$ & $84.95 \pm 0.13$ &  $\textbf{0.0252}\pm 0.0009$ \\ % temp 0.5
			% \hline 
			MAP (SWA) &  $0.4991\pm 0.0041$ & $85.01\pm 0.17$ &  $0.0716\pm 0.0020$ \\ 
			% \hline 
			SWAG & $0.4837\pm 0.0035$ & $84.59 \pm 0.05$ &  $0.0595 \pm 0.0022$ \\ 
			\hline 
		\end{tabular} 
}
\caption{\textbf{Comparisons on STL10 with Monkey class removed}:.}
\label{tab:nll-acc-ece-stl10-pruned}
\end{table*}



\section{CNML Regret} \label{appendix:cnml-regret}

\begin{figure}[t!]
\centering
\begin{subfigure}[t]{0.25\linewidth}
    % \includegraphics[width=\linewidth]{NeuRIPS2019/figures/vgg16_seed1_testdist_compvscorrecness.png}
    \includegraphics[width=\linewidth]{NeuRIPS2019/figures/vgg16_seed1_testdist_compvscorrecness_broken.png}
    \caption{CIFAR10}
    \label{fig:comp-histograms:cifar_comps}
\end{subfigure}%
\begin{subfigure}[t]{.25\linewidth}
    % \includegraphics[width=\linewidth]{NeuRIPS2019/figures/vgg16_seed1_ooddist_compvscorrecness.png}
    \includegraphics[width=\linewidth]{NeuRIPS2019/figures/vgg16_seed1_ooddist_compvscorrecness_broken.png}
    \caption{STL (OOD Data)}
    \label{fig:comp-histograms:stl_comps}
\end{subfigure}%
\begin{subfigure}[t]{0.25\linewidth}
    \includegraphics[width=\linewidth]{NeuRIPS2019/figures/wrn28x10_seed1_testdist_compvscorrectness_broken.png}
    \caption{CIFAR10}
    \label{fig:comp-histograms:cifar_comps_wrn}
\end{subfigure}%
\begin{subfigure}[t]{.25\linewidth}
    \includegraphics[width=\linewidth]{NeuRIPS2019/figures/wrn28x10_seed1_ooddist_compvscorrectness_broken.png}
    \caption{STL (OOD Data)}
    \label{fig:comp-histograms:stl_comps_wrn}
\end{subfigure}%
\caption{Histograms showing the log normalization value $\Phi(x_n)$ (on a logarithmic scale)
for correctly labeled points (blue) and incorrectly labeled points (gold), with VGG16 (left two figures) and WideResNet28x10 (right two figures), on both the in-distribution CIFAR10 test set (a) and the out-of-distribution STL10 images (b). In both cases, we see that, as expected, almost all of the misclassified points have higher values of $\Phi(x_n)$, suggesting this is a useful statistic for assessing classifier confidence with ACNML. Note the breaks in the $y$-scales.}
\label{fig:comp-correctness-hist}
\end{figure}
% \todo{introduce stochastic complexity in unconditional NML, explain it as a notion of complexity, then explain how the conditional one now measures a notion of complexity wrt to a datapoint, representing epistemic uncertainty} 
\todo{shove everything we used to have about $\phi$ in here}
For CNML, the minimax regret is given by the log-normalizer
\begin{equation}
    \Phi_{x^{n-1}, y^{n-1}}(x_n) = \log \sum_{y_n \in \mathcal Y} p_{\hat \theta(x^n, y^n)}(y_n \vert x_n),
\end{equation}
and can serve as a measure of confidence in the prediction made via CNML.
% Intuitively, $\Phi(x_n)$ were high, then that implies that there are labels $y_n$ such that $p_{\hat \theta(x_n, y_n)}$ assigns much higher probability to $y_n$ than $p_{\hat \theta(x^{n-1}, y^{n-1})}$ would, indicating that there are multiple potential labels that are 
Intuitively, if there were different models $p_{\theta}$ that could each assign high probabilities to different proposed labels $y_n$ while maintaining good performance on the train set, $\Phi(x_n)$ would be higher and we should be less confident in the prediction, since multiple labels appear plausible and consistent with our training data, where this notion of consistency is determined by the function class we use.
% Intuitively, if only one label $y_n$ was consistent with the training data, then the maximum likelihood estimators for the other labels would not assign much more weight than the maximum likelihood estimator for just the training set and $\Phi(x_n)$ would be close to 0, while if multiple labels were plausible $\Phi(x_n)$ would be higher.
\citet{Bibas2019DeepNetworks} demonstrate that $\Phi_{x^{n-1}, y^{n-1}}(x_n)$ is a indeed a useful measure of confidence. 
%% This bit on the normalizer seems a bit out of place here; the justification for why it is useful is fairly handwavey.

In \autoref{fig:comp-correctness-hist}, we see that nearly all data points that are incorrectly classified have higher values for the log normalization constant $\Phi(x_n)$, indicating that $\Phi(x_n)$ can be a useful measure of confidence in the models prediction. 

We further assess this in \autoref{fig:comp-reliabilities}, plotting a variant of a reliability diagram to quantitatively see how $\Phi(x_n)$ corresponds to predictive accuracy. We see again that larger values of $\Phi(x_n)$ generally correlate very strongly to decreased accuracy, further reinforcing the hypothesis that this is a reasonable measure of model confidence.

Similar to the reliability diagrams using confidence, for the modified reliability diagrams using $\Phi(x_n)$ in Figure \ref{fig:comp-reliabilities}, we divide into 20 evenly sized bins based on the values of $\Phi(x_n)$.
%% Maybe emphasize that our competitors do not have meaningful normalization constants?
\begin{figure}% {R}{1.0\textwidth}
    \centering\begin{subfigure}[t]{0.5\linewidth}
        \includegraphics[width=\linewidth]{NeuRIPS2019/figures/vgg16_seed1_compreliability.png}
        \caption{VGG16}
        \label{fig:comp-reliability-vgg}
   
    \end{subfigure}%
    \begin{subfigure}[t]{0.5\linewidth}
        \includegraphics[width=\linewidth]{NeuRIPS2019/figures/wrn28x10_seed1_compreliability.png}
        \caption{WideResNet28x10}
        \label{fig:comp-reliability-wrn}
   
    \end{subfigure}%
    \caption{Reliability diagram plotting accuracy against the value of $\log \Phi(x)$. This plot shows that $\Phi(x)$ can be used as a valid measure for the confidence of the ACNML distribution, with larger values of $\Phi(x)$ corrresponding to less accurate predictions.}
    \label{fig:comp-reliabilities}
\end{figure}


==> iclr2020_conference_former_bbl <==
\begin{thebibliography}{3}
\providecommand{\natexlab}[1]{#1}
\providecommand{\url}[1]{\texttt{#1}}
\expandafter\ifx\csname urlstyle\endcsname\relax
  \providecommand{\doi}[1]{doi: #1}\else
  \providecommand{\doi}{doi: \begingroup \urlstyle{rm}\Url}\fi

\bibitem[Bengio \& LeCun(2007)Bengio and LeCun]{Bengio+chapter2007}
Yoshua Bengio and Yann LeCun.
\newblock Scaling learning algorithms towards {AI}.
\newblock In \emph{Large Scale Kernel Machines}. MIT Press, 2007.

\bibitem[Goodfellow et~al.(2016)Goodfellow, Bengio, Courville, and
  Bengio]{goodfellow2016deep}
Ian Goodfellow, Yoshua Bengio, Aaron Courville, and Yoshua Bengio.
\newblock \emph{Deep learning}, volume~1.
\newblock MIT Press, 2016.

\bibitem[Hinton et~al.(2006)Hinton, Osindero, and Teh]{Hinton06}
Geoffrey~E. Hinton, Simon Osindero, and Yee~Whye Teh.
\newblock A fast learning algorithm for deep belief nets.
\newblock \emph{Neural Computation}, 18:\penalty0 1527--1554, 2006.

\end{thebibliography}


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%
\iffalse
\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak
\fi
